Gentrification, displacement, and income trajectory of incumbents

Gentrification is associated with rapid demographic changes within inner-city neighborhoods. While many fear that gentrification drives low-income people from their homes and communities, there is limited evidence of the consequences of these changes. I use Canadian administrative tax files to track the movements of incumbent workers and their income trajectory as their neighborhood gentrifies. I exploit the timing at which neighborhoods gentrify in a matched staggered event-study framework. I find no evidence of displacement effects, even for low socioeconomic status households. In fact, families living in gentrifying neighborhoods are more likely to stay longer. I suggest that this might be related to tenant rights protection laws. When they endogenously decide to leave, low-income families do not relocate to worse neighborhoods. Finally, I find no adverse effects on their income trajectory, suggesting no repercussions on their labor market outcomes.

==> Figures/Balance_table_gentrifiable.tex <==
\caption{Balance table, gentrifiable CT
\label{tab:Bal_table_gent}}
\footnotesize
\onehalfspacing
\begin{center}
\begin{tabular}{lcccc}
\hline \hline
                                & \multicolumn{2}{c}{Mean and sd}                               & \multicolumn{2}{c}{Regression}  \\ 
\textbf{}                       & \multicolumn{1}{l}{Treated} & \multicolumn{1}{l}{Non-treated} & \multicolumn{2}{c}{coefficients} \\[0.1cm] \cline{2-5} 
Median income   growth (\$)     & 987.97                      & 1452.13                         & -464.159*            & 230.191              \\
                                & (3134.41)                     & (2630.10)                         & (259.352)            & (220.112)            \\
                                & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}            & {[}0.075{]}          & {[}0.297{]}          \\
Employment growth               & -.0035                      & 0.0005                           & -0.004               & 0.005                \\
                                & (0.0584)                       & (0.0569)                           & (0.005)              & (0.004)              \\
                                & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}            & {[}0.401{]}          & {[}0.266{]}          \\
Rent growth (\%)                & 0.0753                       & 0.0874                           & -0.012               & -0.002               \\
                                & (0.0931)                       & (0.0992)                           & (0.008)              & (0.008)              \\
                                & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}            & {[}0.153{]}          & {[}0.822{]}          \\
Fraction of low-income growth   & 0.0320                       & 0.0132                           & 0.019**              & -0.009               \\
                                & (0.1074)                       & (0.0982)                           & (0.009)              & (0.006)              \\
                                & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}            & {[}0.031{]}          & {[}0.145{]}          \\
Fraction of college educ growth & 0.0120                       & 0.0261                           & -0.014***            & -0.011***            \\
                                & (0.0375)                       & (0.0308)                           & (0.003)              & (0.003)              \\
                                & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}            & {[}0.000{]}          & {[}0.001{]}          \\[0.2cm]
Controls                        & \multicolumn{1}{l}{}        & \multicolumn{1}{l}{}            & No                   & Yes                  \\ \hline \hline
\end{tabular}
\end{center}
\footnotesize Source: Author's calculations using the Census. \\
Note: The sample includes the 470 census tract x census year included in the main regressions.  Standard errors are reported in parentheses and are clustered at the census tract level. *** $p<0.01$, ** $p<0.05$, * $p<0.1$. P-values are reported in brackets.
Controls include CMA and year FE, distance from CBD and an indicator of whether the tract is gentrifiable.

